ANHALTEN: Cross-Lingual Transfer for German Token-Level Reference-Free Hallucination Detection

Research on token-level reference-free hallucination detection has predominantly focused on English, primarily due to the scarcity of robust datasets in other languages. This has hindered systematic investigations into the effectiveness of cross-lingual transfer for this important NLP application. To address this gap, we introduce ANHALTEN, a new evaluation dataset that extends the English hallucination detection dataset to German. To the best of our knowledge, this is the first work that explores cross-lingual transfer for token-level reference-free hallucination detection. ANHALTEN contains gold annotations in German that are parallel (i.e., directly comparable to the original English instances). We benchmark several prominent cross-lingual transfer approaches, demonstrating that larger context length leads to better hallucination detection in German, even without succeeding context. Importantly, we show that the sample-efficient few-shot transfer is the most effective approach in most setups. This highlights the practical benefits of minimal annotation effort in the target language for reference-free hallucination detection. Aiming to catalyze future research on cross-lingual token-level reference-free hallucination detection, we make ANHALTEN publicly available: https://github.com/janekh24/anhalten

==> 06-related.tex <==
% Tried to make this short and contain some information about the listed paper. Not easy, might have to rewrite
%\vspace{-0.6em}

Despite significant progress, there is a notable gap in token-level reference-free hallucination detection for languages other than English. Research has indicated that diverse models with varied training data can mitigate hallucinations in over 100 language pairs~\citep{guerreiro2023hallucinations}. And the absence of token-level reference-free benchmarks in other languages is crucial, especially for real-time text generation, as fine-grained detection provides immediate feedback for correction~\citep{liu-etal-2022-token}.


% For hallucination detection in the machine translation task, a naturally generated, human-annotated dataset has been released for nine language pairs~\citep{dale-etal-2023-halomi}. Hallucinations in multilingual translation models have been analyzed for over 100 language pairs, finding that more diverse models with different training data can mitigate hallucinations~\citep{guerreiro2023hallucinations}. For the abstractive summarization task, a new multilingual metric has been developed to evaluate faithfulness and detect hallucinations. ~\citep{qiu-etal-2023-detecting}.

% Different approaches to two major types of hallucination detection exist (token-level and sentence-level), which have been reviewed~\citep{luo2024hallucination}. The token-level reference-free hallucination detection task \textsc{HaDes} has been introduced, together with a dataset only in English~\citep{liu-etal-2022-token}. The reference-free sentence and passage-level approach SelfCheckGPT is sample-based and leverages the idea that samples should be similar and consistent if they are correct~\citep{manakul-etal-2023-selfcheckgpt}. Recently, a framework for real-time reference-free hallucination detection that does not require human annotations and instead utilizes the internal states of LLMs has been proposed~\citep{su2024unsupervised}.




% \textcolor{blue}{@Janek}
% Multilingual Hallucination detection for machine translation~\citep{dale-etal-2023-halomi, guerreiro2023hallucinations}, for % summarization focusing on evaluation metrics~\citep{qiu-etal-2023-detecting}
% report?~\citep{luo2024hallucination}: sentence level and token level hallucination detection

% reference-free token level~\citep{liu-etal-2022-token}

% reference-free sentence and passage level~\citep{manakul-etal-2023-selfcheckgpt}

% most recent one~\citep{su2024unsupervised}

% Propose a novel token-level reference-free hallucination detection annotated
% dataset. Additionally, a series of token-level detection models baselines are implemented and
% evaluated on the proposed dataset.
% This work centers on detecting hallucinations at the token-level without relying on groundtruth references. While existing methods often operate at the sentence or document level
% with an oracle reference, these approaches face challenges when ground-truth references
% are unavailable for free-form text generation. In addition, detecting at finer token levels can be crucial for real-time prevention of misleading content as well. This work provides two
% important initial steps towards hallucination detection under this setup. First, the authors
% develop a novel token-level reference-free hallucination detection annotated dataset named
% HADES (HAllucination DEtection dataSet). They then create a series of baseline token-level
% detection models trained on this dataset. These models can detect potential hallucinations
% at the token level without the need for an oracle reference. This approach could be useful in
% real-time applications where ground-truth references may not be readily available.
% To construct the HADES dataset, roughly three steps are followed. First, a large number
% of text segments extracted from English language Wikipedia (English WIKI-40B [13]) using
% BERT [20] are perturbed. In applying this contextual perturbation the authors maintain two
% principles: 1) the fluency and syntactic correctness of the perturbed text should be preserved;
% 2) the perturbed text should be lexically diverse. The text perturbation process is split into
% three operations, namely MASK, REPLACE and RANK. In the MASK step, one word (named
% entity) spans are masked based on a predefined mask ratio. Then, in the REPLACE step, a
% pretrained BERT-base model is leveraged to predict the masked span and replace the span
% with the prediction. All top-k (k=10) samplings are considered as possible candidates as
% this provides a good trade-off between diversity (number of distinct tokens) and coherence
% (number of incoherent perturbations). In the final step, the perturbed text is post-processed
% with a RANK operation as an additional screening step to filter out global incoherence and
% syntactic issues. In the end, the authors collect around 1M perturbed text segments in the pool
% after contextual perturbation. One thing to note is that not all of these contain hallucination, as the BERT model can generate factual information given that it is pretrained on a rich open
% web corpus.
% After the initial data perturbation, the authors use human annotation for the labeling process.
% Here, they use a so-called “model-in-the-loop” procedure to annotate a challenging subset, as
% human annotation is prohibitively expensive at this scale. The annotation process is split into
% several rounds. For each round, they first retrain a hallucination detection model (initialized
% with BERT) on the annotated instances from the previous rounds. This model is used to select
% the next batch of data to be annotated from the remaining unlabeled data. In total, after
% accumulating annotations for several rounds, they obtain 12,719 instances with 71,226 HITS
% from judges. They conduct 14 rounds of annotation, increasing the annotation scale with
% each round (ranging from around 200 instances/round to around 4000 instances/round). Out
% of 12,719 annotated instances, 10,954 instances reached consensus among judges and are
% included in the HADES dataset. The dataset is split into train, validation and test sets with sizes
% of 8754, 1000, 1200 respectively. In the final dataset, “hallucination” cases slightly outnumber
% “not hallucination” cases, with a ratio of 54.5%/45.5%.
% Methodology-wise, this work proposes a series of baseline methods based on pretrained
% transformer models, including BERT [20], GPT-2 [40], XLNet [54] and RoBERTa [60]. These
% transformer-based models can potentially leverage context or embedded world knowledge to
% detect self-contradictory or anti-commonsense content. Specifically, for an input text segment
% and a target token, the model predicts binary hallucination labels for the given text spans. The
% authors propose two different settings: online and offline. In the online setting, the model
% can only access the unidirectional preceding context, which simulates on-the-fly generation.
% While in the offline setting, it is assumed that generation is complete, so the the model is able
% to perceive the bidirectional context. The results are shown in Figure 3.1 and Figure 3.2 for
% online and offline settings respectively.
% One thing worth mentioning is that for the baseline transformer-based detectors, longer
% context length tends to result in a better performance. The authors run BERT-large detection
% model with different context lengths and characterize its performance in both online and
% offline settings. Starting from the target words, they set a fixed size (5/10/20/40/80/160)
% context window and truncate all text beyond this window. As the context window enlarges, the
% model performance grows rapidly when context length is smaller than 80, and then gradually
% converges. This observation highlights the importance of context in hallucination detection
% using the detectors in this work. Therefore, one should pay attention to the use case of the
% HADEs detection model that it might underperform when the text length is not sufficiently
% long.




==> table/03-translate_train.tex <==
\setlength{\tabcolsep}{6.2 pt}
\begin{table*}[h]
\centering
\footnotesize{
\begin{tabular}{l ccccc ccc ccc}
\toprule
& & & & & & \multicolumn{3}{c}{\textbf{Not Hallucination}} & \multicolumn{3}{c}{\textbf{Hallucination}} \\ \cmidrule(l{.4em}){7-9}\cmidrule(l{.5em}){10-12}
\textbf{Model} & \textbf{Setting} & \textbf{Accuracy $\uparrow$} & \textbf{G-Mean $\uparrow$} & \textbf{BS $\downarrow$} & \textbf{AUC $\uparrow$} & \textbf{P $\uparrow$} & \textbf{R $\uparrow$} & \textbf{F1 $\uparrow$} & \textbf{P $\uparrow$} & \textbf{R $\uparrow$} & \textbf{F1 $\uparrow$} \\ \midrule

mBERT & offline & 64.54 & 63.76 & 22.61 & 70.46 & 66.97 & 62.61 & 63.99 & 63.44 & 66.57 & 64.35 \\
mBERT & online & 64.78&63.66 &22.66 & 71.11& 69.43& 57.66& 62.05& 62.55&72.28 & 66.45\\\midrule
XLMR & offline & 66.42 & 64.13 & 21.30 & 73.80 & 66.69& 72.44&67.84 &69.98 &60.08 &62.91 \\ 
XLMR & online & 67.66&66.55 & 21.02& 73.20&65.66 &77.66 &71.13 &70.86 & 57.13&63.19 \\
  \bottomrule
\end{tabular}%
}
%\vspace{-0.6em}
\caption{Translate-train transfer results.}
\label{tab:eval_result_tranlate_train}
%\vspace{-0.7em}
\end{table*}
